RCHOL: Randomized Cholesky Factorization for Solving SDD Linear Systems

We introduce a randomized algorithm, namely RCHOL, to construct an approximate Cholesky factorization for a given Laplacian matrix (a.k.a., graph Laplacian). From a graph perspective, the exact Cholesky factorization introduces a clique in the underlying graph after eliminating a row/column. By randomization, RCHOL only retains a sparse subset of the edges in the clique using a random sampling developed by Spielman and Kyng. We prove RCHOL is breakdown-free and apply it to solving large sparse linear systems with symmetric diagonally dominant matrices. In addition, we parallelize RCHOL based on the nested dissection ordering for shared-memory machines. We report numerical experiments that demonstrate the robustness and the scalability of RCHOL. For example, our parallel code scaled up to 64 threads on a single node for solving the 3D Poisson equation, discretized with the 7-point stencil on a $1024\times 1024 \times 1024$ grid, a problem that has one billion unknowns.

==> sdd.bak.tex <==
\subsection{SDD Matrix} \label{s:sdd2}

Given a non-singular irreducible SDD matrix $A \in \mathbb{R}^{N \times N}$, let $A_d, A_n, A_p  \in \mathbb{R}^{N \times N}$ contain the diagonal, the negative off-diagonal and the positive off-diagonal entries of $A$, respectively. In this section, we focus on the case when $A_p$ is not zero, i.e., $A$ contains at least one positive off-diagonal entry. For the analysis in this section, we need to consider two different scenarios:
\begin{enumerate} [leftmargin=4.5cm,label=\textbf{S.\arabic*}]
\item \label{s1}
$\forall \, i, \, a_{ii} = \sum_{j\not=i} |a_{ij}|$
\item \label{s2}
$\exists \, i, \, a_{ii} > \sum_{j\not=i} |a_{ij}|$
\end{enumerate}


\begin{lemma} \label{l:sdd}
Matrix $F \triangleq A_d+A_n-A_p$ is an irreducible Laplacian matrix when \cref{s1} holds, or an irreducible SDDM matrix when \cref{s2} holds.
\end{lemma}
\begin{proof} 

$F$ is SDD with only negative off-diagonal entries and is irreducible because it has the same sparsity as $A$. 
 With regard to scenarios in \cref{s1,s2}:
\begin{enumerate} %[label=\textbf{S.\arabic*}]
\item 
$F$ is a Laplacian matrix, as can be easily verified.
\item
%Without loss of generality, assume $f_{11} = \alpha - \sum_{j\not=1} f_{1j}$, where $\alpha>0$, and $f_{ii} = - \sum_{j\not=i} f_{ij}$ when $i\not=1$. For any non-zero vector $x \in \mathbb{R}^{N}$, consider the quadratic form
%\[
%x^\top F x = \alpha x_1^2 + \sum_{f_{ij} \not= 0} (-f_{ij}) (x_i - x_j)^2 > 0
%\]
$F$ is an SDDM matrix, becasue $F$ is positive definite based on the Gershgorin circle theorem.
\end{enumerate}
\end{proof}


\begin{theorem} \label{t:sdd}
Solving a non-singular irreducible SDD linear system $Ax=b$, where there exists $a_{ij} > 0$ and $i\not=j$, is equivalent to solving %the following linear system
\begin{equation} \label{e:ext2}
\tilde{A} \, y
=
\begin{pmatrix}
b \\
-b
\end{pmatrix},
\end{equation}
where 
\begin{equation} \label{e:sdde}
\tilde{A}
\triangleq
\begin{pmatrix}
A_d+A_n & -A_p \\
-A_p & A_d+A_n
\end{pmatrix}
\end{equation}
is an SDD matrix with only negative off-diagonal entries, and 
%\begin{equation}
$
y = 
\begin{pmatrix}
x \\
-x
\end{pmatrix}
$
%\end{equation}
is the only solution that is orthogonal to $\text{span}\{\bone\}$ (null space of $\tilde{A}$ if \cref{s1} holds).
\end{theorem}
\begin{proof}
It is straightforward to verify \cref{e:sdde} is SDD with only negative off-diagonal entries. Assume 
$
y = 
\begin{pmatrix}
x_1 \\
-x_2
\end{pmatrix}
$
is the solution of \cref{e:ext2}, i.e.,
\begin{align*}
(A_d+A_n) x_1 + A_p x_2 = b \\
 A_p x_1 + (A_d+A_n) x_2 = b 
\end{align*}
If we sum the above two equations we obtain
\[
x_1 + x_2 =  2 x
\]
If we take the difference of the above two equations we obtain (recall $F$ in \cref{l:sdd})
\[
F \, (x_1 - x_2) = 0
\]
Consider the two scenarios \cref{s1,s2}. According to \cref{l:sdd},
\begin{enumerate} %[label=\textbf{S.\arabic*}]
\item
When $F$ is an irreducible Laplacian matrix. We have $x_1 - x_2 \in \text{span}\{\bone\}$, so the solution of \cref{e:ext2} is
$
y = 
\begin{pmatrix}
x \\
-x
\end{pmatrix}
+ 
\text{span}\{\bone\}.
$
\item
When $F$ is an irreducible SDDM matrix. We obtain $x_1 = x_2 = x$.
\end{enumerate}
\end{proof}


